A Few Teacher Steps Go a Long Way: Efficient SFT Data Collection for LLM Agents

DAgger-style supervised finetuning (SFT) combines full teacher demonstrations with teacher continuations of partial student rollouts, providing supervision on contexts the student encounters. We study how to allocate the teacher-inference budget on these on-policy (OP) continuations after initial behavior cloning (BC). One existing collection recipe runs the teacher to termination and retains only successful continuations (OP-Success). Since rejected outputs still incur teacher-inference costs, we compare this recipe with shorter continuations without outcome filtering (OP-Short), and with continuing only failed learner rollouts while retaining successful continuations (OP-Critical). We evaluate these choices against acquiring additional full demonstrations, tracking total teacher-inference cost separately from retained training tokens. Across HotpotQA, ALFWorld, and OpenThoughts-TB-Dev, teacher continuations improve the accuracy-cost tradeoff over scaling full demonstrations. On HotpotQA and OpenThoughts-TB-Dev, OP-Short surpasses the strongest tested BC baseline while reducing estimated teacher-inference cost by 20% and 83%, respectively, and on ALFWorld five-step continuations cut teacher tokens by 22% relative to full continuations with little accuracy loss. Controlled HotpotQA ablations show that by focusing on failed student rollouts, OP-Critical achieves comparable accuracy to OP-Success with 30% lower estimated teacher-inference cost and 36% fewer retained training tokens. Compute-matched comparisons with reinforcement learning and on-policy distillation further support brief teacher continuations as an efficient and lightweight post-training recipe.

==> tables/hotpotqa_checkpoints/op_critical.tex <==

\HPSweep{$1$}{3}{%
  \HPScore{45.4}{43.6}{47.2} & \HPScore{50.5}{48.7}{52.3} & \HPBest{51.8}{50.0}{53.6} & \HPNA & \HPNA & \HPNA & \HPNA%
}{51.8}

\HPSweep{$1$}{5}{%
  \HPScore{45.9}{44.1}{47.7} & \HPScore{50.7}{48.9}{52.5} & \HPBest{52.6}{50.8}{54.4} & \HPScore{52.1}{50.3}{53.9} & \HPScore{52.0}{50.2}{53.8} & \HPNA & \HPNA%
}{52.6}

\HPSweep{$1$}{7}{%
  \HPScore{46.0}{44.2}{47.8} & \HPScore{51.1}{49.3}{52.9} & \HPScore{50.9}{49.2}{52.8} & \HPScore{52.3}{50.5}{54.1} & \HPSelected{53.3}{51.5}{55.1} & \HPScore{52.0}{50.1}{53.8} & \HPBest{53.3}{51.6}{55.1}%
}{53.3}

\HPRecipeBreak

\HPSweep{$2$}{3}{%
  \HPScore{46.6}{44.8}{48.4} & \HPBest{51.7}{49.9}{53.5} & \HPScore{51.1}{49.3}{52.9} & \HPNA & \HPNA & \HPNA & \HPNA%
}{51.7}

\HPSweep{$2$}{5}{%
  \HPScore{47.5}{45.7}{49.3} & \HPScore{50.2}{48.4}{52.0} & \HPScore{52.7}{50.9}{54.5} & \HPScore{52.8}{51.0}{54.6} & \HPBest{53.6}{51.8}{55.4} & \HPNA & \HPNA%
}{53.6}

\HPSweep{$2$}{7}{%
  \HPScore{47.5}{45.7}{49.3} & \HPScore{50.6}{48.9}{52.5} & \HPScore{52.7}{51.0}{54.6} & \HPScore{52.2}{50.3}{54.0} & \HPScore{53.6}{51.8}{55.4} & \HPScore{52.6}{50.8}{54.4} & \HPSelected{54.3}{52.6}{56.1}%
}{54.3}

\HPRecipeBreak

\HPSweep{$3$}{3}{%
  \HPScore{47.4}{45.6}{49.2} & \HPScore{51.5}{49.7}{53.3} & \HPBest{52.0}{50.2}{53.8} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.0}

\HPSweep{$3$}{5}{%
  \HPScore{47.5}{45.7}{49.3} & \HPScore{49.5}{47.7}{51.3} & \HPScore{52.8}{51.0}{54.6} & \HPScore{52.7}{50.9}{54.5} & \HPBest{53.3}{51.5}{55.1} & \HPNA & \HPNA%
}{53.3}

\HPSweep{$3$}{7}{%
  \HPScore{47.7}{45.9}{49.5} & \HPScore{50.5}{48.7}{52.2} & \HPScore{52.7}{50.9}{54.5} & \HPScore{53.2}{51.3}{55.0} & \HPScore{53.0}{51.2}{54.9} & \HPScore{52.8}{51.0}{54.6} & \HPSelected{53.4}{51.6}{55.2}%
}{53.4}

\HPRecipeBreak

\HPSweep{$5$}{3}{%
  \HPScore{46.3}{44.5}{48.1} & \HPBest{52.1}{50.3}{53.9} & \HPScore{51.5}{49.7}{53.3} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.1}

\HPSweep{$5$}{5}{%
  \HPScore{46.4}{44.6}{48.2} & \HPScore{51.8}{50.0}{53.6} & \HPScore{52.3}{50.5}{54.1} & \HPBest{53.0}{51.2}{54.8} & \HPScore{52.7}{50.9}{54.5} & \HPNA & \HPNA%
}{53.0}

\HPSweep{$5$}{7}{%
  \HPScore{47.7}{45.9}{49.5} & \HPScore{50.7}{48.9}{52.6} & \HPScore{52.1}{50.3}{53.9} & \HPScore{52.6}{50.8}{54.4} & \HPSelected{53.6}{51.9}{55.5} & \HPScore{52.4}{50.7}{54.2} & \HPScore{53.5}{51.7}{55.4}%
}{53.6}


==> tables/hotpotqa_checkpoints/op_short.tex <==

\HPSweep{$1$}{3}{%
  \HPScore{49.6}{47.8}{51.4} & \HPScore{51.9}{50.0}{53.7} & \HPBest{52.1}{50.4}{53.9} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.1}

\HPSweep{$1$}{5}{%
  \HPScore{48.5}{46.7}{50.3} & \HPScore{51.6}{49.8}{53.4} & \HPScore{54.0}{52.2}{55.8} & \HPScore{52.8}{51.0}{54.6} & \HPSelected{54.5}{52.8}{56.3} & \HPNA & \HPNA%
}{54.5}

\HPSweep{$1$}{7}{%
  \HPScore{48.5}{46.7}{50.3} & \HPScore{50.5}{48.8}{52.3} & \HPScore{53.3}{51.4}{55.1} & \HPScore{53.4}{51.6}{55.2} & \HPScore{53.2}{51.5}{55.0} & \HPScore{53.4}{51.6}{55.2} & \HPBest{53.9}{52.1}{55.7}%
}{53.9}

\HPRecipeBreak

\HPSweep{$2$}{3}{%
  \HPScore{49.7}{47.9}{51.6} & \HPScore{51.7}{49.8}{53.4} & \HPBest{52.7}{50.9}{54.5} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.7}

\HPSweep{$2$}{5}{%
  \HPScore{49.3}{47.5}{51.0} & \HPScore{52.0}{50.2}{53.8} & \HPScore{52.4}{50.6}{54.2} & \HPSelected{54.1}{52.3}{55.9} & \HPScore{53.1}{51.3}{54.9} & \HPNA & \HPNA%
}{54.1}

\HPSweep{$2$}{7}{%
  \HPScore{48.3}{46.5}{50.1} & \HPScore{52.2}{50.4}{54.0} & \HPScore{53.1}{51.3}{55.0} & \HPScore{53.1}{51.3}{54.9} & \HPScore{52.6}{50.8}{54.4} & \HPBest{53.7}{51.9}{55.5} & \HPScore{53.5}{51.7}{55.3}%
}{53.7}

\HPRecipeBreak

\HPSweep{$3$}{3}{%
  \HPScore{49.3}{47.5}{51.1} & \HPBest{53.3}{51.5}{55.2} & \HPScore{53.1}{51.3}{54.9} & \HPNA & \HPNA & \HPNA & \HPNA%
}{53.3}

\HPSweep{$3$}{5}{%
  \HPScore{49.3}{47.5}{51.1} & \HPScore{51.8}{50.0}{53.6} & \HPBest{53.7}{51.9}{55.5} & \HPScore{53.2}{51.4}{55.0} & \HPScore{53.4}{51.6}{55.2} & \HPNA & \HPNA%
}{53.7}

\HPSweep{$3$}{7}{%
  \HPScore{50.3}{48.5}{52.1} & \HPScore{51.2}{49.4}{53.0} & \HPScore{53.6}{51.8}{55.5} & \HPScore{54.0}{52.2}{55.8} & \HPSelected{54.3}{52.5}{56.1} & \HPScore{54.2}{52.4}{56.0} & \HPScore{53.3}{51.5}{55.1}%
}{54.3}

\HPRecipeBreak

\HPSweep{$5$}{3}{%
  \HPScore{51.4}{49.6}{53.2} & \HPScore{52.0}{50.3}{53.8} & \HPBest{52.5}{50.7}{54.3} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.5}

\HPSweep{$5$}{5}{%
  \HPScore{49.9}{48.1}{51.8} & \HPScore{52.0}{50.2}{53.8} & \HPScore{53.1}{51.3}{54.9} & \HPScore{53.6}{51.8}{55.4} & \HPSelected{54.5}{52.7}{56.3} & \HPNA & \HPNA%
}{54.5}

\HPSweep{$5$}{7}{%
  \HPScore{50.5}{48.7}{52.3} & \HPScore{52.4}{50.6}{54.2} & \HPScore{54.2}{52.4}{56.0} & \HPScore{52.8}{51.0}{54.6} & \HPBest{54.5}{52.7}{56.3} & \HPScore{53.7}{51.9}{55.5} & \HPScore{53.5}{51.7}{55.3}%
}{54.5}


==> tables/hotpotqa_checkpoints/op_success.tex <==

\HPSweep{$1$}{3}{%
  \HPScore{47.5}{45.7}{49.3} & \HPScore{50.7}{48.9}{52.5} & \HPBest{52.0}{50.2}{53.8} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.0}

\HPSweep{$1$}{5}{%
  \HPScore{47.9}{46.1}{49.7} & \HPScore{50.7}{48.9}{52.5} & \HPScore{51.9}{50.1}{53.7} & \HPScore{53.0}{51.2}{54.8} & \HPBest{53.5}{51.7}{55.3} & \HPNA & \HPNA%
}{53.5}

\HPSweep{$1$}{7}{%
  \HPScore{47.3}{45.5}{49.1} & \HPScore{49.3}{47.5}{51.1} & \HPScore{52.0}{50.2}{53.9} & \HPSelected{54.2}{52.5}{56.1} & \HPScore{52.4}{50.6}{54.2} & \HPScore{53.3}{51.5}{55.1} & \HPScore{52.2}{50.4}{54.0}%
}{54.2}

\HPRecipeBreak

\HPSweep{$2$}{3}{%
  \HPScore{48.7}{46.9}{50.5} & \HPScore{50.9}{49.1}{52.7} & \HPBest{52.0}{50.2}{53.8} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.0}

\HPSweep{$2$}{5}{%
  \HPScore{48.4}{46.6}{50.2} & \HPScore{50.0}{48.2}{51.8} & \HPScore{53.4}{51.6}{55.2} & \HPScore{52.0}{50.2}{53.8} & \HPSelected{54.4}{52.6}{56.2} & \HPNA & \HPNA%
}{54.4}

\HPSweep{$2$}{7}{%
  \HPScore{49.1}{47.4}{51.0} & \HPScore{50.1}{48.3}{51.9} & \HPBest{53.2}{51.4}{55.0} & \HPScore{52.6}{50.8}{54.4} & \HPScore{52.3}{50.5}{54.1} & \HPScore{53.0}{51.2}{54.8} & \HPScore{53.2}{51.5}{55.0}%
}{53.2}

\HPRecipeBreak

\HPSweep{$3$}{3}{%
  \HPScore{48.8}{47.0}{50.7} & \HPBest{52.7}{51.0}{54.6} & \HPScore{52.5}{50.7}{54.3} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.7}

\HPSweep{$3$}{5}{%
  \HPScore{49.7}{47.9}{51.5} & \HPScore{51.3}{49.6}{53.1} & \HPScore{53.5}{51.7}{55.3} & \HPSelected{54.2}{52.4}{56.1} & \HPScore{53.5}{51.7}{55.4} & \HPNA & \HPNA%
}{54.2}

\HPSweep{$3$}{7}{%
  \HPScore{49.0}{47.2}{50.8} & \HPScore{51.8}{50.0}{53.7} & \HPScore{52.5}{50.7}{54.3} & \HPScore{53.6}{51.8}{55.4} & \HPBest{54.0}{52.2}{55.8} & \HPScore{52.9}{51.1}{54.7} & \HPScore{53.6}{51.8}{55.4}%
}{54.0}

\HPRecipeBreak

\HPSweep{$5$}{3}{%
  \HPScore{50.4}{48.6}{52.2} & \HPScore{51.1}{49.3}{52.9} & \HPBest{53.1}{51.3}{54.9} & \HPNA & \HPNA & \HPNA & \HPNA%
}{53.1}

\HPSweep{$5$}{5}{%
  \HPScore{48.8}{47.0}{50.6} & \HPScore{51.7}{49.9}{53.5} & \HPScore{54.0}{52.2}{55.8} & \HPScore{53.4}{51.6}{55.2} & \HPSelected{54.2}{52.4}{56.0} & \HPNA & \HPNA%
}{54.2}

\HPSweep{$5$}{7}{%
  \HPScore{49.1}{47.3}{50.9} & \HPFail & \HPScore{53.0}{51.2}{54.8} & \HPScore{53.2}{51.4}{55.0} & \HPScore{53.3}{51.5}{55.1} & \HPScore{53.0}{51.2}{54.8} & \HPBest{53.6}{51.8}{55.4}%
}{53.6}


==> tables/hotpotqa_checkpoints/pure_bc.tex <==

\HPSweep{$1k\,q\!\times\!1$}{3}{%
  \HPScore{44.5}{42.8}{46.3} & \HPScore{49.0}{47.2}{50.8} & \HPBest{49.7}{47.9}{51.5} & \HPNA & \HPNA & \HPNA & \HPNA%
}{49.7}

\HPSweep{$1k\,q\!\times\!1$}{5}{%
  \HPScore{44.9}{43.1}{46.7} & \HPScore{49.1}{47.3}{50.9} & \HPScore{51.2}{49.4}{53.0} & \HPBest{51.5}{49.7}{53.3} & \HPBest{51.5}{49.7}{53.3} & \HPNA & \HPNA%
}{51.5}

\HPSweep{$1k\,q\!\times\!1$}{7}{%
  \HPScore{45.4}{43.6}{47.2} & \HPScore{49.3}{47.5}{51.1} & \HPScore{51.7}{50.0}{53.6} & \HPScore{51.1}{49.3}{52.9} & \HPScore{51.7}{49.8}{53.5} & \HPSelected{52.1}{50.3}{53.9} & \HPScore{51.8}{50.0}{53.7}%
}{52.1}

\HPRecipeBreak

\HPSweep{$1k\,q\!\times\!2$}{3}{%
  \HPScore{47.6}{45.9}{49.5} & \HPScore{51.3}{49.4}{53.1} & \HPBest{51.7}{49.9}{53.5} & \HPNA & \HPNA & \HPNA & \HPNA%
}{51.7}

\HPSweep{$1k\,q\!\times\!2$}{5}{%
  \HPScore{48.6}{46.8}{50.4} & \HPScore{50.0}{48.2}{51.8} & \HPSelected{52.2}{50.4}{54.0} & \HPScore{51.2}{49.4}{53.0} & \HPScore{51.0}{49.2}{52.8} & \HPNA & \HPNA%
}{52.2}

\HPSweep{$1k\,q\!\times\!2$}{7}{%
  \HPScore{48.0}{46.3}{49.8} & \HPScore{50.3}{48.5}{52.2} & \HPScore{51.0}{49.3}{52.9} & \HPBest{51.8}{50.1}{53.7} & \HPScore{51.7}{49.9}{53.5} & \HPScore{51.5}{49.7}{53.3} & \HPScore{50.9}{49.2}{52.8}%
}{51.8}

\HPRecipeBreak

\HPSweep{$1k\,q\!\times\!3$}{3}{%
  \HPScore{48.7}{46.9}{50.5} & \HPScore{50.2}{48.3}{52.1} & \HPBest{51.8}{50.0}{53.6} & \HPNA & \HPNA & \HPNA & \HPNA%
}{51.8}

\HPSweep{$1k\,q\!\times\!3$}{5}{%
  \HPScore{48.5}{46.7}{50.3} & \HPScore{51.6}{49.9}{53.5} & \HPScore{52.0}{50.2}{53.8} & \HPBest{52.5}{50.7}{54.4} & \HPScore{52.4}{50.6}{54.2} & \HPNA & \HPNA%
}{52.5}

\HPSweep{$1k\,q\!\times\!3$}{7}{%
  \HPScore{48.6}{46.8}{50.4} & \HPScore{50.5}{48.7}{52.4} & \HPScore{52.0}{50.2}{53.8} & \HPScore{51.3}{49.6}{53.2} & \HPScore{52.0}{50.2}{53.9} & \HPScore{52.3}{50.5}{54.1} & \HPSelected{52.6}{50.8}{54.3}%
}{52.6}

\HPRecipeBreak

\HPSweep{$1k\,q\!\times\!4$}{3}{%
  \HPScore{50.7}{48.9}{52.6} & \HPBest{52.4}{50.6}{54.2} & \HPScore{52.3}{50.5}{54.1} & \HPNA & \HPNA & \HPNA & \HPNA%
}{52.4}

\HPSweep{$1k\,q\!\times\!4$}{5}{%
  \HPScore{49.6}{47.8}{51.4} & \HPScore{51.6}{49.8}{53.4} & \HPBest{53.4}{51.6}{55.2} & \HPScore{52.9}{51.1}{54.7} & \HPScore{52.3}{50.5}{54.1} & \HPNA & \HPNA%
}{53.4}

\HPSweep{$1k\,q\!\times\!4$}{7}{%
  \HPScore{50.0}{48.2}{51.9} & \HPScore{50.7}{48.9}{52.5} & \HPScore{52.1}{50.4}{53.9} & \HPScore{53.2}{51.4}{55.0} & \HPScore{53.2}{51.4}{55.0} & \HPScore{52.7}{50.9}{54.6} & \HPSelected{53.9}{52.2}{55.7}%
}{53.9}

